Risk Assessment of Stealthy Attacks on Uncertain Control Systems

In this article, we address the problem of risk assessment of stealthy attacks on uncertain control systems. Considering data injection attacks that aim at maximizing impact while remaining undetected, we use the recently proposed output-to-output gain to characterize the risk associated with the impact of attacks under a limited system knowledge attacker. The risk is formulated using a well-established risk metric, namely the maximum expected loss. Under this setups, the risk assessment problem corresponds to an untractable infinite non-convex optimization problem. To address this limitation, we adopt the framework of scenario-based optimization to approximate the infinite non-convex optimization problem by a sampled non-convex optimization problem. Then, based on the framework of dissipative system theory and S-procedure, the sampled non-convex risk assessment problem is formulated as an equivalent convex semi-definite program. Additionally, we derive the necessary and sufficient conditions for the risk to be bounded. Finally, we illustrate the results through numerical simulation of a hydro-turbine power system.

==> 3_Omniscient.tex <==
To recall, solving a robust problem \eqref{uncertain:system} is computationally intensive since the set $\Omega$ is a continuum. One way to solve this problem is to adopt the scenario-based approach \cite{calafiore2007probabilistic}. The scenario-based approach states that: By sampling an uncertainty set densely, the solution obtained by solving the sampled version of the optimization problem is approximately feasible for the original optimization problem. By using this framework, we determine an approximate solution to the optimization problem \eqref{uncertain:system} in this section and provide probabilistic guarantees on the original robust optimization problem.

\subsection{Discrete uncertainty set}

To begin with, we consider an uncertainty set $\Omega$ which is discrete. The results of this section is the basis for addressing a continuous uncertainty set. For brevity, given a sampled uncertainty $\delta_i \in \Omega$, we define $\tilde{\Sigma}_{p,i} \triangleq ({A}_{cl,i}, {B}_{cl,i}, {C}_{p,i}, {D}_{p,i})$ and  $\tilde{\Sigma}_{r,i} \triangleq ({A}_{cl,i}, {B}_{cl,i}, {C}_{r,i}, {D}_{r,i})$ with $y_p(\delta_i)=y_{pi},y_r(\delta_i)=y_{ri}$ and $x(\delta_i)=x_{i}$ as the outputs and states of $\tilde{\Sigma}_{p,i}$ and  $\tilde{\Sigma}_{r,i}$ correspondingly. For such an isolated uncertainty, the optimization problem \eqref{eqq4} can be rewritten as

\begin{equation}\label{pp1}
\begin{aligned}
 ||\tilde{\Sigma}(\delta_i)||_{\ell_{2e},y_p \leftarrow y_r}^2 &\triangleq  \sup_{a_i \in \ell_{2e}}\; X^A(a_i,\delta_i)\\
 & \begin{aligned}
  =\sup_{a_i \in \ell_{2e}} & \Vert y_{p,i}\Vert_{\ell_2}^2\\
\textrm{s.t.} \; & \Vert y_{r,i}\Vert_{\ell_2}^2 \leq 1,x_i[\infty]=0,
\end{aligned}
\end{aligned}
\end{equation}
where $a_i$ is the attack vector corresponding to the uncertainty $\delta_i$. Using the Lagrange dual function, the non-convex optimization problem \eqref{pp1} can be rewritten into a convex dual problem. This equivalency is depicted in the following lemma.

\begin{lemma}\label{dual_OA}
The optimization problems \eqref{pp1} and \eqref{t5} are equivalent.
\begin{equation}\label{t5}
\begin{aligned}
||\tilde{\Sigma}(\delta_i)||_{\ell_{2e},y_p \leftarrow y_r}^2 = \inf_{\gamma_i \geq 0 } \; & \gamma_i \\
\textrm{s.t.} \; & ||y_{p,i}||^2_{\ell_{2}} - \gamma_i||y_{r,i}||_{\ell_2}^2 \leq 0, \forall a_i \in \ell_{2e}\\
& x_i[0]=0,x_i[\infty]=0,
\end{aligned}
\end{equation}
\end{lemma}
\begin{proof}
The proof is postponed to Appendix \ref{proof_remark}.
\end{proof}

The constraint of the optimization problem \eqref{t5} lies in the signal space which is infinite-dimensional. It would be convenient if the inequality is in the form of a finite-dimensional matrix inequality. To this end, following \cite{Truncated} (also see Appendix \ref{diss_app} \textit{Proposition  \ref{prop1}, $3)$}), the constraint of \eqref{t5} can be characterized as a matrix inequality such that the following conditions are equivalent:
\begin{enumerate}
    \item Given that $x_i[0]=x_i[\infty]=0$, it holds $\forall a_i \in \ell_{2e}$ that \[||y_{p,i}||_{\ell_2}^2 - \gamma_i ||y_{r,i}||_{\ell_2}^2 \leq 0. \]
    \item $\exists P_i=P_i^T \; \text{s.t.}\; M(\gamma_i,\delta^i,P_i) \preceq 0,$ where
\end{enumerate}
\begin{multline*}
M (\gamma_i,\delta^i,P_i) \triangleq 
\begin{bmatrix} A_{cl,i}^TP_iA_{cl,i}-P_i & A_{cl,i}^TP_iB_{cl,i} \\ B_{cl,i}^TP_iA_{cl,i} & B_{cl,i}^TP_iB_{cl,i} \end{bmatrix} 
+\\
\begin{bmatrix}
C_{p,i}^T\\
D_{p,i}^T
\end{bmatrix}
\begin{bmatrix}
C_{p,i} & D_{p,i}
\end{bmatrix} - \gamma_i
\begin{bmatrix}
C_{r,i}^T\\
D_{r,i}^T
\end{bmatrix}
\begin{bmatrix}
C_{r,i} & D_{r,i}
\end{bmatrix}.
\end{multline*}
Using this equivalency, \eqref{t5} is reformulated as a convex SDP in the following lemma.
\begin{lemma}\label{lemm1}
The optimization problem \eqref{t5} and the following optimization problem are equivalent.
\begin{equation}\label{s2}
\begin{aligned}
||\tilde{\Sigma}(\delta_i)||_{\ell_{2e},y_p \leftarrow y_r}^2 = \min_{\gamma_i \geq 0 ,P_i = P_i^T} \; & \gamma_i \\
\textrm{s.t.} \; & M (\gamma_i,\delta^i,P_i) \preceq 0 \end{aligned}
\end{equation}
$\hfill\square$
\end{lemma}

Next, we discuss the the conditions for boundedness of $||\tilde{\Sigma}(\delta_i)||_{\ell_{2e},y_p \leftarrow y_r}^2$ in the following lemma.

\begin{lemma}[Boundedness]\label{bound_OA_single}
Consider the closed-loop system \eqref{system:CL:uncertain} with an uncertainty $\delta_i$ which is known to the adversary. Then, the optimal value of \eqref{s2} is bounded if and only if one of the following condition hold:
\begin{enumerate}
    \item The system $\tilde{\Sigma}_{r,i}$ has no zeros on the unit circle.
    \item The zeros on the unit circle of the system $\tilde{\Sigma}_{r,i}$ (including multiplicity and input direction) are also zeros of $\tilde{\Sigma}_{p,i}$.
\end{enumerate}
\end{lemma}
\begin{proof}
See Appendix \ref{bound_1}.
\end{proof}

In words, the above lemma states that the attack impact caused by an omniscient adversary on the closed-loop \eqref{system:CL:uncertain} with an uncertainty $\delta_i$ is bounded if either, there does not exist an attack vector which makes the output $y_r$ identically zero, or for all attack vectors which yields $y_r$ identically $0$, it also yields $y_p$ identically zero. To this end, we have formulated the results on characterizing the attack impact by a convex SDP and the condition for its boundedness when the uncertainty set is discrete. These results are the basis for addressing a continuous uncertainty set. Next, the approach discussed in this section is extended to the risk assessment framework when considering a continuum of uncertainties.

\subsection{Continuous uncertainty set}

The optimization problem \eqref{s2} can be directly extended to solve \eqref{uncertain:system} only when we consider a discrete set $\Omega$. But the optimization problem \eqref{uncertain:system} that we intend to solve has a set $\Omega$ which is a continuum. Using the framework of scenario-based reliability estimation \cite{calafiore2007probabilistic}, $\Omega$ can be approximated with a finite set. With this framework of scenario-based reliability estimation, we revisit \eqref{uncertain:system} in the theorem below. 

\begin{theorem}\label{Thm1}
Let $\epsilon_1 \in (0,1)$ represent the accuracy with which the probability operator $\mathbb{P}_{\Omega}$ in \eqref{uncertain:system} is to be approximated. Let $\beta_1 \in (0,1)$ represent the confidence with which the accuracy $\epsilon_1$ is guaranteed, i.e.,
\[ \mathbb{P}\{ \vert \mathbb{P}_{\Omega}(||\tilde{\Sigma}(\delta)||_{\ell_{2e},y_p \leftarrow y_r}^2 \leq \gamma ) - \hat{\mathbb{P}}_{N_1} \vert \geq\epsilon_1\} \leq \beta_1.\]
Here $ \hat{\mathbb{P}}_{N_1}$ represents the approximation of the probability operator $\mathbb{P}_{\Omega}$ in \eqref{uncertain:system} defined as
\[
\hat{\mathbb{P}}_{N_1} \triangleq \frac{1}{N_1}\sum_{i=1}^{N_1}\mathbb{I}\left( ||\tilde{\Sigma}(\delta_i)||_{\ell_{2e},y_p \leftarrow y_r}^2 \leq \gamma \right),
\]
where
\begin{equation}\label{sam1}
N_1 \geq \frac{1}{2\epsilon_1^2}\text{log}\frac{2}{\beta_1}.
\end{equation}
Then, the $\text{VaR}_{\beta}$ defined in \eqref{uncertain:system} can be obtained with an accuracy $\epsilon_1$ and confidence $\beta_1$ by solving
\begin{equation}\label{problem:decoupled}
\begin{aligned}
\min & \;\;\gamma\\
\textrm{s.t.} \quad & \frac{1}{N_1} \sum_{i=1}^{N_1} \mathbb{I}\left( \gamma_i \leq \gamma \right) \geq 1-\beta,
\end{aligned}
\end{equation}
where $\mathbb{I}$ is the indicator function. The value of  $\gamma_i\;\forall i \in \{1,\dots, N_1\}$ is obtained by solving the convex optimization problem \eqref{s2}.
\end{theorem}
\begin{proof}
See Appendix \ref{App1}
\end{proof}

\textit{Theorem \ref{Thm1}} states that, to solve \eqref{problem:decoupled}, one could solve the optimization problem \eqref{s2} or equivalently \eqref{t5} for $N_1$ unique realizations of the uncertainty. Since strong duality holds between \eqref{t5} and \eqref{pp1}, the optimal value of the dual optimization problem \eqref{problem:decoupled} indeed provides the VaR$_{\beta}$ with an accuracy $\epsilon_1$. Next, by extending \textit{Lemma \ref{bound_OA_single}}, the condition for boundedness of \eqref{problem:decoupled} is stated in the following lemma.

\begin{lemma}[Boundedness]\label{bound_OA_multi}
Consider $N_1$ independent and identically distributed (i.i.d) realizations of the closed-loop system \eqref{system:CL:uncertain}, each with an uncertainty $\delta_i$. The optimal value of \eqref{problem:decoupled} with these $N_1$ system realizations is bounded if and only if the optimal value of \eqref{s2} is bounded for at least $\left \lceil{N_1(1-\beta)}\right \rceil $ system realizations. 
\end{lemma}
\begin{proof}
Necessity: Let us multiply both sides of the constraint of \eqref{problem:decoupled} by $N_1$. Then, for a bounded solution $\gamma_{OA}$ to exist, we require that
\begin{equation}
\sum_{i=1}^{N_1} \mathbb{I}\left( \gamma_i \leq \gamma_{OA} , \; \forall a_i \in \ell_{2e}\right) \geq N_1-N_1\beta,
\end{equation}
should hold with a bounded $\gamma_{OA}$. This is satisfied only if $
\lceil N_1(1-\beta)\rceil$ values of the set $\{\gamma_i\}_{i=1,\dots,N_1}$ are bounded.\\
Sufficiency: Assume that the values of the set $\{\gamma_i\}_{i=1,\dots,N_1}$, for the first $\left \lceil N_1(1-\beta)\right \rceil$ realizations is bounded and is unbounded for the other realizations. Let us choose $\gamma_{OA} = \max_{i=1,\dots,\lceil N_1(1-\beta) \rceil} \gamma_i$. Substituting the definition of $\gamma_i, \gamma_{OA}$ in the constraint of \eqref{problem:decoupled} yields
\begin{align*}
&\frac{1}{N_1}\left\{\sum_{i=1}^{\lceil N_1(1-\beta)\rceil} \mathbb{I}\left( \gamma_i \leq \gamma_{OA} \right) + \sum_{i=\lceil N_1(1-\beta)\rceil +1}^{N_1} \mathbb{I}\left( \gamma_i \leq \gamma_{OA} \right) \right\} \\
&=\frac{1}{N_1}\left\{ \lceil N_1(1-\beta) \rceil + 0 \right\} \geq 1-\beta.
\end{align*}
Thus, there exists a bounded $\gamma_{OA}$ which satisfies the constraint of \eqref{problem:decoupled}. This concludes the proof.
\end{proof}

The interpretation of \textit{Lemma \ref{bound_OA_multi}} is that the system operator tolerates a fraction ($\beta \times 100 \%$) of cases where the impact \eqref{s2} is unbounded. Conversely, even-though the impact is unbounded for certain elements of the uncertainty set, the risk assessed by the system operator will still be bounded. This allows the system operator to be less pessimistic. 

In this section, we have discussed a scenario-based approach to determine the VaR$_{\beta}$. The risk assessment problem was posed as a convex SDP. However, the number of optimization problems necessary to determine the risk is $N_1$. Next, we discuss an approach to solve the optimization problem \eqref{w1}.
